Does Vector Quantization Fail in Spatio-Temporal Forecasting? Exploring a Differentiable Sparse Soft-Vector Quantization Approach

Spatio-temporal forecasting is crucial in various fields and requires a careful balance between identifying subtle patterns and filtering out noise. Vector quantization (VQ) appears well-suited for this purpose, as it quantizes input vectors into a set of codebook vectors or patterns. Although VQ has shown promise in various computer vision tasks, it surprisingly falls short in enhancing the accuracy of spatio-temporal forecasting. We attribute this to two main issues: inaccurate optimization due to non-differentiability and limited representation power in hard-VQ. To tackle these challenges, we introduce Differentiable Sparse Soft-Vector Quantization (SVQ), the first VQ method to enhance spatio-temporal forecasting. SVQ balances detail preservation with noise reduction, offering full differentiability and a solid foundation in sparse regression. Our approach employs a two-layer MLP and an extensive codebook to streamline the sparse regression process, significantly cutting computational costs while simplifying training and improving performance. Empirical studies on five spatio-temporal benchmark datasets show SVQ achieves state-of-the-art results, including a 7.9% improvement on the WeatherBench-S temperature dataset and an average mean absolute error reduction of 9.4% in video prediction benchmarks (Human3.6M, KTH, and KittiCaltech), along with a 17.3% enhancement in image quality (LPIPS). Code is publicly available at https://github.com/Pachark/SVQ-Forecasting.

==> sections/1_introduction.tex <==

\section{Introduction}



Spatio-temporal forecasting~\cite{spatio-temporal-survey:2022} has board applications in many domains including environment, climate, transportation, etc. Many traditional methods relying on feature engineering have been studied in the past several decades. Recently, deep learning models are becoming more popular~\cite{spatio-temporal-survey:2022}. However, as more applications (e.g., weather forecasting) arise, it calls for deep models to accurately predict future dynamics with precise spatial and temporal resolutions.
%%%The field of self-supervised learning has undergone amazing progress in the past few years, with well-known algorithms such as masked modeling~\cite{maskgit} and contrastive learning~\cite{simclr}. Most studies are limited to modeling static images, even when the original data source is video. which is critical to applications such as weather forecasting, remains relatively underexplored. These tasks pose considerable challenges, demanding models to accurately predict future dynamics with precise spatial and temporal resolutions.



% While recurrent models such as ConvLSTM~\cite{convlstm}, PredRNN~\cite{predrnn}, and E3D-LSTM~\cite{e3dlstm} have been the mainstay, latest studies have shifted towards non-recurrent models~\cite{SimVP,simvpv2,tau} for better accuracy and efficiency. 
Despite the various forms of spatio-temporal forecasting approaches, such as the use of graph neural network (GNN) models for unevenly resolved data, our work concentrates on grid-based datasets, one of the most widely adopted structures in the field. Within this context, we address a primary challenge: how to finely balance the preservation of important details against the need to filter out irrelevant noise, thereby enhancing the generalized performance of forecasting models. Although vector quantization (VQ) is effective in reducing noises by constraining latent patterns to a clustered codebook, it is usually limited in preserving the diversity of input patterns, making it suboptimal for spatial-temporal forecasting. We performed a comprehensive suite of experiments, the results of which indicate that, contrary to expectations, nearly all sota VQ methods we examined did not enhance the accuracy of a basic weather forecasting model as shown in Table \ref{tab:ablation_vq_method}. This outcome may provide insight into the infrequent application of VQ techniques in spatial-temporal prediction tasks. 

\begin{figure}[H]
  \centering
  \includegraphics[width=0.9\linewidth]{graphs/codebook_tsne_vq.pdf}
  \includegraphics[width=0.9\linewidth]{graphs/vector_quantization_comparison4.png}
  \caption{{\bf Hard-VQ vs Soft-VQ and cookbook visualization} \small Bottom-Left:hard-VQ sample. Bottom-right:soft-VQ sample.Top-Left: VQ updated by k-means clustering . Top Right: SVQ with randomly initialized, frozen or learnable codebook. }
  \label{fig:codebook_tsne_vq}
  \vskip -0.25in
\end{figure}
%Two methods are trained on WeatherBench-S temperature dataset with the same codebook size (1024).and exponential moving average as described in~\cite{vqvae}
To address this limitation of VQ, we propose a {\bf S}parse regression-based {\bf V}ector {\bf Q}uantization ({\bf SVQ}) method. By associating each vector to multiple codes from a large codebook, it is able to cover diverse visual patterns; by introducing a sparse regularization mechanism in the regression model, we effectively filter out noise and thus ensure a good generalized performance. As shown in Figure \ref{fig:codebook_tsne_vq}, our proposed SVQ method exhibits a more uniform distribution of quantized vectors compared to VQ, indicating that SVQ is able to preserve more diverse and fine-grained information from the original inputs than VQ. 

Despite employing a series of vectors for representation instead of a single codebook vector, regression-based vector quantization(soft-VQ) remains true to the foundational aspects of the technique, as shown in Figure \ref{fig:codebook_tsne_vq}, It still quantizes input vectors into a finite set of discrete levels, utilizing a dynamic codebook-like structure. The key process of mapping input data to representative vectors is maintained, but with the added sophistication of regression models that adaptively combine vectors for a more accurate representation. This method preserves the essence of vector quantization—efficiently compressing and approximating data—while enhancing its ability to capture complex patterns within the input space.

To address the high computational cost of sparse regression, which
scales quadratically with codebook size, we approximate the sparse regression model with a MLP model and a large codebook. It not only dramatically simplifies the computation, but more importantly, makes SVQ differentiable and thus easy to train. We emphasize the importance of differentiability of SVQ for its success in spatial-temporal forecasting. Our experiments reveal that lookup-based VQ methods can substantially increase prediction error, despite some employing a residual design that theoretically should perform on par with or better than non-VQ cases. This suggests the ``straight-through" estimator, a non-differentiable component of VQ, may be a major factor behind VQ's underperformance. In particular, the non-differentiable operator such as argmin or lookup introduces errors into gradient estimation of all modules preceding the quantization module, consequently undermining prediction accuracy. In contrast, our proposed SVQ is differentiable and easy to compute accurate gradients for training. We finally note that SVQ also differs from traditional VQ methods by not relying on intricate models to construct the prior distribution of codes, such as the GPT-style model in VQGAN~\cite{vqgan} or the BERT-style model in MaskGIT~\cite{maskgit}.


%because, according to our empirical study, non-differentiability of traditional VQ methods may be the key to their failure
%\newpage

%This is because our experiments show that a lookup-based VQ method often result in a significant increase in prediction error even with a residual based design which in nature should be at least as good as VQ-free case, indicating that the ``straight-through'' estimator, a non-differential part of VQ, may contribute largely to the poor performance of VQ. 

%\textcolor{red}{In section ~\ref{sec:position_vq}, our experiments demonstrate that employing a lookup-based learned codebook, traditional VQ performs poorly, often resulting in a significantly increased prediction error. This sheds light on why noise reduction techniques of this sort are seldom utilized in spatiotemporal forecasting tasks. One contributing factor may be the ``straight-through estimator" method, which is non-differentiable due to the argmin or lookup operation. This limitation introduces errors into the gradient flow of all modules preceding the quantization module, consequently undermining prediction accuracy. In contrast, our proposed SVQ leverages a differentiable approach that not only preserves the capability to generate robust features but also facilitates a smooth learning curve, ultimately directly enhancing forecasting performance, without relying on intricate priors like those in VQGAN~\cite{vqgan} or MaskGIT~\cite{maskgit}. This enhancement can be attributed to the representation capability of quantization module.}

Besides differentiability, there are two interesting properties of the proposed SVQ scheme. First, according to our empirical study, we find that with large enough codebook size, we can freeze the randomly initialized codebook without sacrificing any performance, making SVQ potentially more efficient for training. Secondly, unlike lookup-based methods, SVQ allows for both positive and negative weights, enhancing the ability to add or subtract patterns to improve representational power.

Finally, despite its simplification, our experiments across multiple real-world benchmark datasets—including weather forecasting, traffic flow prediction, and video forecasting, demonstrate the superior performance of our SVQ method. In WeatherBench-S temperature forecasting benchmark, it improves the prior SOTA method by 7.9\%. For video prediction across renowned datasets—Human3.6M, KTH, and KittiCaltech—SVQ not only achieves a consistent 9.4\% reduction in MAE but also enhances perceptual quality, evidenced by a 17.3\% lower LPIPS score. These results highlight SVQ's versatility and superior accuracy in diverse spatial-temporal prediction scenarios.

%\textcolor{red}{Our approach showcases two main attributes. Firstly, we align our model with Vector Quantization (VQ), distinguishing it from typical external memory networks~\cite{lee2021video} by using a potentially fixed random matrix as our ``cookbook." This represents a major shift, as our continuous regression-based VQ successfully encodes original images with random vectors. We find that with a sufficiently large codebook size, the performance of a frozen codebook is on par with that of a carefully trained one, bypassing the need to learn codebook from training data. Secondly, unlike lookup-based methods, our regression-based technique allows for both positive and negative weights, enhancing the ability to add or subtract patterns to improve representational power.}

%\textcolor{red}{The principal innovation of our work is to demonstrate that sparse regression, despite its inherent complexity, can be effectively approximated using a two-layer Multilayer Perceptron (MLP) coupled with a randomly fixed or learnable ``cookbook". This significantly enhances computational efficiency. We underscore the versatility of the proposed SVQ method, which can be integrated with any non-recurrent backbone architecture to boost prediction accuracy. Our experiments across multiple real-world benchmark datasets—including weather forecasting, traffic flow prediction, and video forecasting—unequivocally validate the efficacy of our SVQ method.}


% In short, the main contributions of this work are outlined as follows:
% \begin{itemize}
%     \itemsep0em 
%     \item Our continuous regression-based VQ encodes original images with random vectors, eliminating the need for learning from training data. Notably, we find that when codebook size is large, a large-sized, frozen randomly-initialized codebook performs comparably to a carefully learned codebook.
%     \item Our regression-based quantization module, endowed with strong representational capacity, enhances forecasting performance directly, without relying on intricate prior models such as the GPT-style model in VQGAN~\cite{vqgan} or the BERT-style model in MaskGIT~\cite{maskgit}.
%     \item We propose an effective approximation of complex sparse regression through a two-layer Multilayer Perceptron (MLP) and a fixed random or a learnable codebook, thereby significantly improving computational efficiency.
%     \item Our regression-based approach uniquely permits both positive and negative weights, thereby increasing the flexibility to add or subtract patterns and enhancing representational power.
% \end{itemize}

==> sections/7_efficient_representation.tex <==
\section{Efficient Utilize of Cookbook Using Sparse Regression}
\label{sec:comp_svq_cluster}
To understand the difference between sparse regression-based quantization scheme and clustering-based quantization scheme, we measure the number of codes that we need in order to approximate any vector within an unit ball $\mathcal{B}$ with error less than $\delta$. We denote this number by $T(\mathcal{B}, \delta)$. As indicated by the theorem below, using spare regression, $T(\mathcal{B}, \delta)$ can be reduced from $O(1/\delta^d)$ to $O(1/\delta^p)$, with $p \ll d$ for high dimensional vectors. 
\begin{theorem}
\label{theorem}
$T(\mathcal{B}, \delta)$ for the clustering-based method is at least $1/\delta^d$, while $T(\mathcal{B},\delta)$ for sparse regression can be $(4d/\delta)^p$, with 
\[
p \geq \max\left(3, \frac{\log(4/\delta)}{\log\log(2d/\varepsilon)}\right), 
\]
as long as the non-zero elements used by sparse regression is at least $
    \frac{4d}{\delta \left(\log C + p\log (4d) - (p+1)\log \delta \right)}.
$
\end{theorem}
\begin{proof}
\renewcommand{\qedsymbol}{}
To bound $T(\mathcal{B}, \delta)$ for the clustering method, we use the covering number for a unit ball $\mathcal{B}$, requiring at least $1/\delta^d$ code vectors to approximate any vector within error $\delta$. Considering $Ug$, with $U = (u_1, \ldots, u_m)$, $u_k \sim \N(0, I_d/m)$, and $g \in \Delta_s$ an $s$-sparse unit vector, we have:
\[
\Pr\left(\|UU^{\top} - I\|_2 \geq \gamma \right) \leq 2d\exp\left(-\frac{m\gamma^2}{3d}\right),
\]
implying
\[
\|UU^{\top} - I\|_2 \leq \Delta := \sqrt{\frac{d}{m}\log\frac{2d}{\varepsilon}}
\]
with probability at least $1 - \varepsilon$. Thus, $\|g' - g\|_2 \geq (1+\Delta)^{-1} \|Ug - Ug'\|_2$. With the $s$-sparse unit vector covering number bounded by $(Cm/s\delta)^s$, we obtain:
\[
\left(\frac{Cm}{s\delta}\right)^s \geq \left(1 + \frac{2}{\delta}\right)^d(1+\Delta)^d,
\]
By choosing $m = (4d/\delta)^p$, we have
\[
(1+\Delta)^d \leq \exp\left(d\Delta\right) \leq e,
\]
yielding $s\log(C'm/\delta) \geq 2d/\delta + s\log s$, given $C' = Ce$. 

As $s \geq 4d/[\delta(\log C + p\log(4d) - (p+1)\log\delta)]$, it is easy to verify that $s\log s \leq 2d/\delta$, leading to $m \geq (4d/\delta)^p$.
\end{proof}

% \begin{proof}
% \renewcommand{\qedsymbol}{}
% To bound $T(\mathcal{B}, \delta)$ for the clustering method, we directly use the covering number result for an unit ball, i.e. in order to approximate any vector in a unit ball $\mathcal{B}$ within an error $\delta$, you need at least $1/\delta^d$ code vectors. To bound $T(\mathcal{B}, \delta)$, we consider $Ug$, where $U = (u_1, \ldots, u_m)$ includes randomly sampled vectors, with each $u_k$ sampled from $\N(0, I_d/m)$ and $g \in \Delta_s$ is an unit vector with $s$ non-zero elements. Since 
% \[
% \Pr\left(|UU^{\top} - I|_2 \geq \gamma \right) \leq 2d\exp\left(-\frac{m\gamma^2}{3d}\right),
% \]
% we have, with a probability $1 - \varepsilon$, 
% \[
%     |UU^{\top} - I|_2 \leq \Delta:=\sqrt{\frac{d}{m}\log\frac{2d}{\varepsilon}}.
% \]
% Thus, with a probability $1 - \varepsilon$, we have for any $g$ and $g'$
% \[
% |g' - g|_2 \geq \frac{1}{1+\Delta} |Ug - Ug'|.
% \]
% Since the covering number for $s$-sparse unit vector is upper bounded by $(Cm/s\delta)^s$, using the fact that packing number upper bounds the covering number, we know that to approximate any vector in the unit ball $\mathcal{B}$, we need
% \[
% \left(\frac{C m}{s\delta}\right)^s \geq \left(1 + \frac{2}{\delta}\right)^d(1+\Delta)^d.
% \]
% By choosing $m = (4d/\delta)^p$, we have
% \[
% (1 + \Delta)^d \leq \exp\left(d\Delta\right) \leq e
% \]
% and therefore
% \[
% \left(\frac{C' m}{s\delta}\right)^s \geq \left(1 + \frac{2}{\delta}\right)^d,
% \]
% where $C' = Ce$. It leads to 
% \[
% s\log\frac{C'm}{\delta} \geq \frac{2d}{\delta} + s\log s.
% \]
% Since 
% \[
% s \geq \frac{4d}{\delta\left(\log C + p\log(4d) - (p+1)\log\delta\right)}
% \]
% % \vspace{2mm}
% it is easy to verify that $s\log s \leq 2d/\delta$, leading to 
% \[
% m \geq \left(\frac{4d}{\delta}\right)^p.
% \]
% % \vspace{-0.5mm}
% \end{proof}

==> tables/tab_ablation.tex <==
\begin{table*}
\centering
\caption{SVQ ablation studies on WeatherBench-S temperature dataset. We ablate important designs based on the default setting: SVQ with 10000 codebook size, learnable codebook, and MAE loss.}
% \vskip 0.15in
\begin{center}
\begin{tabular}{cc}
\begin{minipage}[c]{0.4\textwidth}

\centering

\begin{tabular}{c|cc}
\toprule
Module &MSE$\downarrow$ & MAE$\downarrow$ \\
\midrule
SimVP (MSE loss)& 1.1308 & 0.6633  \\
SimVP+MAE loss&	1.1265 &	0.6509 \\
SimVP+SVQ+MSE loss&	1.0994 &	0.6527 \\
SimVP+SVQ+MAE loss&	\textbf{1.0182} &	\textbf{0.6109} \\
\bottomrule
\end{tabular}
\caption*{(a) \textbf{Module ablation}. The joint use of SVQ and MAE loss is significant.}
\end{minipage}

\hspace{1cm}
\begin{minipage}[c]{0.4\textwidth}
\centering

\begin{tabular}{c|c|cc}
\toprule
Learnability & Codebook size &	MSE$\downarrow$ & MAE$\downarrow$\\
\midrule
\multirow{3}{*}{Frozen} &10\textasciicircum{}1 & 1.0696 & 0.6227 \\
 &10\textasciicircum{}3 & 1.0436 & 0.6198 \\
 &10\textasciicircum{}4 & 1.0230 & 0.6131 \\
\midrule
\multirow{3}{*}{Learnable} &10\textasciicircum{}1 & 1.0492 & 0.6200 \\
 &10\textasciicircum{}3 & 1.0479 & 0.6182 \\
 &10\textasciicircum{}4 & \textbf{1.0182} &	\textbf{0.6109}\\
\bottomrule
\end{tabular}
\caption*{(b) \textbf{Codebook size and learnablity}. Increasing codebook size improves performance. Difference between learnable and frozen codebook narrows when significantly increasing codebook size.}

\end{minipage}
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{cc}

\begin{minipage}[c]{0.5\textwidth}
\centering
\begin{tabular}{c|c|ccc}
\toprule
Learnability & Initialization & MSE$\downarrow$ & MAE$\downarrow$ & Kurtosis\\
\midrule
\multirow{5}{*}{Frozen} & kaiming uniform & 1.0230 & 0.6131 & 1.596 \\
&xavier uniform & 1.0479 &0.6179 &1.544 \\
&sparse(sparsity=0.9) &1.0498&0.6183 &4.165 \\
&trunc normal & 1.0497 & 0.6166 &1.582 \\
&orthogonal &1.0343&0.6170 &1.561 \\
\midrule
\multirow{5}{*}{Learnable}& kaiming uniform & 1.0182 & 0.6109 & 7.213\\
&xavier uniform & 1.0464 &0.6176 &31.931\\
&sparse(sparsity=0.9) & 1.0342 &0.6160 &41.558\\
&trunc normal & 1.0307 &0.6161 & 4.236\\
&orthogonal & 1.0302 &0.6131 & 35.774\\
\bottomrule
\end{tabular}
\caption*{(c) \textbf{Codebook initialization method}. Learnable codebook slightly improves performance across all initialization methods. Kaiming uniform achieves the best results.}
\end{minipage}


\hspace{1cm}


\begin{minipage}[c]{0.4\textwidth}
\centering
\begin{tabular}{c|cc}
\toprule
Method &MSE$\downarrow$ & MAE$\downarrow$ \\
\midrule
VQ\cite{vqvae}& 1.8544 & 0.8963 \\
Residual VQ\cite{residualvq}& 1.8882 & 0.9237 \\
Grouped Residual VQ\cite{groupresidualvq}& 1.1737 & 0.6747 \\
Multi-headed VQ\cite{multiheadvq}&	1 &	1 \\
Residual Finite Scalar Quantization\cite{fsq}& 1.3192 & 0.7505 \\
Lookup Free Quantization (LFQ)\cite{lookupfreevq} &	1 &	1 \\
Residual LFQ\cite{lookupfreevq}& 1.2806 & 0.7281\\
SVQ& \textbf{1.0182} &	\textbf{0.6109}\\
\bottomrule
\end{tabular}
\caption*{(d) \textbf{Vector quantization method}. SVQ directly improves the downstream forecasting performance.}
\end{minipage}

\end{tabular}


\end{center}
\label{tab_ablation}
\end{table*}

==> tables/tab_ablation_balance.tex <==
\begin{table}
\caption{\small  {\bf Predition MSE} on WeatherBench-S temperature dataset with Grouped Residual VQ (GRVQ) and SVQ.}
\begin{center}
\begin{small}
% \begin{sc}
\scalebox{0.8}{
\begin{tabular}{c|ccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{Codebook size} \\
\cmidrule{2-6}
 & 16 & 64 & 256 & 1024 & 4096 \\
\midrule
GRVQ& 1.463&1.233 &1.211&1.174& 1.206\\
SVQ& 1.065& 1.060& 1.046& 1.040&1.028\\
\bottomrule
\end{tabular}
}
\label{tab:ablation_balance}
% \end{sc}
\end{small}
\end{center}
\end{table}

==> tables/tab_noise.tex <==
\begin{table}[H]
\centering
% \captionsetup{font=small} 
\caption{{\bf Noise injection analysis:} The proportion of injected noise is indicated by $\eta$. We present MSE and MAE, and their percentage increase over baseline without artificial noise.}
\begin{center}
% \begin{small}
% \begin{sc}
\scalebox{0.9}{
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2}{*}{Noise proportion} & \multicolumn{2}{c|}{MSE}            & \multicolumn{2}{c}{MAE}           \\
\cmidrule{2-5}
                                  & w/o SVQ          & w SVQ           & w/o SVQ         & w SVQ           \\
\midrule
$\eta$=0                                 & 1.105            & 1.018           & 0.6567          & 0.6109          \\
$\eta$=10\%                              & 1.386(+25.4\%)   & 1.051(+3.2\%)  & 0.7702(+17.3\%) & 0.6269(+2.6\%)  \\
$\eta$=20\%                              & 1.554(+40.7\%)   & 1.196(+17.5\%)  & 0.8282(+26.1\%) & 0.6710(+9.8\%)  \\
$\eta$=30\%                              & 1.750(+58.4\%)   &      1.255(+23.2\%)  & 0.8821(+34.3\%) &   0.6953(+13.8\%) \\
$\eta$=40\%                              & 2.081(+88.3\%)   & 1.568(+54.0\%)    & 1.0031(+52.7\%) &  0.7973(+30.5\%)   \\
$\eta$=50\%                              & 2.646(+139.4\%) & 1.529(+50.2\%) & 1.1339(+72.7\%) & 0.7881(+29.0\%)\\
\bottomrule
\end{tabular}
\label{tab:noise}
}
% \end{sc}
% \end{small}
\end{center}
%\vspace{-5mm}
\end{table}


==> tables/tab_sup_significance.tex <==
\begin{table*}[h]
\centering
\caption{Statistical significance of models on the WeatherBench-M dataset.}
\begin{center}
\vskip -0.1in
\begin{small}
\scalebox{0.65}{
% \begin{sc}
\begin{tabular}{cc|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c|}{Variable}&\multicolumn{2}{c|}{Temperature}&\multicolumn{2}{c|}{Humidity}&\multicolumn{2}{c|}{Wind Component}&\multicolumn{2}{c}{Total Cloud Cover}\\
% \midrule
\midrule
\multicolumn{2}{c|}{Model}&MSE$\downarrow$ & MAE$\downarrow$ & MSE$\downarrow$ & MAE$\downarrow$ &MSE$\downarrow$ & MAE$\downarrow$ & MSE$\downarrow$ & MAE$\downarrow$ \\
\midrule
\multicolumn{2}{c|}{SimVP (w/o VQ)}& 4.833$\pm$0.031 & 1.5246$\pm$0.0077 & 340.06$\pm$0.44 & 12.738$\pm$0.030 & 24.535$\pm$0.076 & 3.4882$\pm$0.0086 & 25.332$\pm$0.052  & 3.4509$\pm$0.0052 \\
\multicolumn{2}{c|}{SimVP+SVQ (Frozen)} &4.427$\pm$0.017 &1.4160$\pm$0.0051 &360.15$\pm$0.55 & 12.445$\pm$0.024 & 23.915$\pm$0.098 & 3.4078$\pm$0.0033 & 24.968$\pm$0.126 & 3.4117$\pm$0.0032 \\
\multicolumn{2}{c|}{SimVP+SVQ (Learnable)} &4.433$\pm$0.021 &1.4164$\pm$0.0054 &360.53$\pm$0.81 & 12.449$\pm$0.013 & 23.908$\pm$0.062 & 3.4060$\pm$0.0029 & 24.983$\pm$0.115 & 3.4095$\pm$0.0038 \\
\bottomrule
\end{tabular}
\label{tab:sup_significance}
}
% \end{sc}
\end{small}
\end{center}
\vskip -0.2in
\end{table*}



==> tables/tab_sup_significance_t2m.tex <==
\begin{table}[H]
\centering
\caption{Statistical significance of models on the WeatherBench-S temperature dataset.}
\begin{center}
\begin{small}
\scalebox{0.65}{
% \begin{sc}
\begin{tabular}{cc|cc}
\toprule
\multicolumn{2}{c|}{Model}&MSE$\downarrow$ & MAE$\downarrow$ \\
\midrule
\multicolumn{2}{c|}{SimVP (w/o VQ)}& 1.105$\pm$0.043 & 0.6567$\pm$0.0185 \\
\multicolumn{2}{c|}{SimVP+SVQ (Frozen)} &1.023$\pm$0.007 &0.6131$\pm$0.0050 \\
\multicolumn{2}{c|}{SimVP+SVQ (Learnable)} &1.018$\pm$0.009 &0.6109$\pm$0.0064 \\
\bottomrule
\end{tabular}
\label{tab:sup_significance_t2m}
}
% \end{sc}
\end{small}
\end{center}
\vskip -0.2in
\end{table}



==> tables/tab_sup_significance_taxibj.tex <==
\begin{table}[H]
\centering
\caption{Statistical significance of models on the TaxiBJ dataset.}
\begin{center}
\begin{small}
\scalebox{0.65}{
% \begin{sc}
\begin{tabular}{cc|cccc}
\toprule
\multicolumn{2}{c|}{Model}&MSE$\downarrow$ & MAE$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ \\
\midrule
\multicolumn{2}{c|}{SimVP (w/o VQ)}& 0.3246$\pm$0.0173 & 15.03$\pm$0.26 & 0.9844$\pm$0.0008 & 39.71$\pm$0.11 \\
\multicolumn{2}{c|}{SimVP+SVQ (Frozen)} &0.3171$\pm$0.0056 &14.68$\pm$0.03 & 0.9848$\pm$0.0001 & 39.83$\pm$0.01 \\
\multicolumn{2}{c|}{SimVP+SVQ (Learnable)} &0.3191$\pm$0.0020 &14.64$\pm$0.02 & 0.9849$\pm$0.0002 & 39.86$\pm$0.02 \\
\bottomrule
\end{tabular}
\label{tab:sup_significance_taxibj}
}
% \end{sc}
\end{small}
\end{center}
\vskip -0.2in
\end{table}

==> tables/tab_weatherbench_hmv.tex <==

\begin{table}[H]
\centering
% \captionsetup{font=small} 
\caption{MAE comparison for SimVP and SVQ on WeatherBench-HMV (The first 55 channels).}
\begin{center}
% \vskip -0.2in
\begin{small}
% \begin{sc}
\scalebox{1}{
\begin{tabular}{c|c|c|c|c}
\toprule
Channel  & SimVP (w/o VQ) & SimVP+SVQ (Frozen) & SimVP+SVQ (Learnable) & Improvement \\
\midrule
u10      & 2.1557         & 2.0849             & 2.0757                & 3.7\%      \\
v10      & 2.1613         & 2.1101             & 2.1117                & 2.4\%      \\
t2m      & 2.5603         & 2.4089             & 2.2799                & 11.0\%     \\
tisr     & 1.13E+05       & 32640              & 30756                 & 72.7\%     \\
tcc      & 0.22906        & 0.22028            & 0.22316               & 3.8\%      \\
tp       & 0.000147       & 9.96E-05           & 9.96E-05              & 32.1\%     \\
z\_50    & 371.19         & 268.81             & 269.45                & 27.6\%     \\
z\_100   & 333.31         & 243.12             & 245.07                & 27.1\%     \\
z\_150   & 339.15         & 265.88             & 267.14                & 21.6\%     \\
z\_200   & 376.12         & 303.11             & 302.84                & 19.5\%     \\
z\_250   & 404.46         & 340.07             & 338.73                & 16.3\%     \\
z\_300   & 404.8          & 347.96             & 347.64                & 14.1\%     \\
z\_400   & 357.33         & 314.15             & 313.48                & 12.3\%     \\
z\_500   & 309.93         & 272.9              & 270.52                & 12.7\%     \\
z\_600   & 276.35         & 241.09             & 237.15                & 14.2\%     \\
z\_700   & 252.58         & 218.67             & 215.86                & 14.5\%     \\
z\_850   & 229.2          & 203.88             & 203.05                & 11.4\%     \\
z\_925   & 229            & 208.52             & 206.46                & 9.8\%      \\
z\_1000  & 242.2          & 220.18             & 219.18                & 9.5\%      \\
pv\_50   & 3.97E-06       & 2.93E-06           & 2.92E-06              & 26.3\%     \\
pv\_100  & 1.44E-06       & 1.32E-06           & 1.33E-06              & 7.8\%      \\
pv\_150  & 9.72E-07       & 8.42E-07           & 8.44E-07              & 13.4\%     \\
pv\_200  & 1.00E-06       & 8.64E-07           & 8.50E-07              & 15.0\%     \\
pv\_250  & 1.05E-06       & 9.77E-07           & 9.73E-07              & 7.7\%      \\
pv\_300  & 8.51E-07       & 7.88E-07           & 8.00E-07              & 7.4\%      \\
pv\_400  & 3.61E-07       & 3.42E-07           & 3.41E-07              & 5.6\%      \\
pv\_500  & 2.35E-07       & 2.28E-07           & 2.28E-07              & 3.1\%      \\
pv\_600  & 3.89E-07       & 3.31E-07           & 3.32E-07              & 14.8\%     \\
pv\_700  & 6.97E-07       & 5.30E-07           & 5.27E-07              & 24.4\%     \\
pv\_850  & 8.81E-07       & 7.70E-07           & 7.62E-07              & 13.6\%     \\
pv\_925  & 1.00E-06       & 9.66E-07           & 9.58E-07              & 4.6\%      \\
pv\_1000 & 1.40E-06       & 1.35E-06           & 1.34E-06              & 4.5\%      \\
r\_50    & 1.9046         & 1.2558             & 1.391                 & 34.1\%     \\
r\_100   & 7.6728         & 6.0793             & 6.3087                & 20.8\%     \\
r\_150   & 9.6361         & 8.4854             & 8.7663                & 11.9\%     \\
r\_200   & 14.653         & 13.175             & 14.435                & 10.1\%     \\
r\_250   & 19.433         & 18.728             & 18.964                & 3.6\%      \\
r\_300   & 20.066         & 19.791             & 19.851                & 1.4\%      \\
r\_400   & 19.78          & 19.375             & 19.356                & 2.1\%      \\
r\_500   & 19.155         & 18.876             & 18.825                & 1.7\%      \\
r\_600   & 18.208         & 17.981             & 17.938                & 1.5\%      \\
r\_700   & 17.216         & 17.041             & 17.055                & 1.0\%      \\
r\_850   & 14.586         & 15.379             & 14.691                & -0.7\%     \\
r\_925   & 10.086         & 9.613              & 9.6737                & 4.7\%      \\
r\_1000  & 7.5008         & 8.0927             & 7.2911                & 2.8\%      \\
q\_50    & 9.03E-08       & 7.40E-08           & 7.55E-08              & 18.1\%     \\
q\_100   & 1.97E-07       & 1.87E-07           & 1.87E-07              & 5.3\%      \\
q\_150   & 1.10E-06       & 1.10E-06           & 1.08E-06              & 2.1\%      \\
q\_200   & 6.68E-06       & 6.48E-06           & 6.39E-06              & 4.3\%      \\
q\_250   & 2.38E-05       & 2.24E-05           & 2.26E-05              & 5.7\%      \\
q\_300   & 5.61E-05       & 5.30E-05           & 5.40E-05              & 5.5\%      \\
q\_400   & 0.000181       & 0.000174           & 0.000177              & 3.9\%      \\
q\_500   & 0.000375       & 0.000364           & 0.000362              & 3.4\%      \\
q\_600   & 0.000592       & 0.000557           & 0.000553              & 6.6\%      \\
q\_700   & 0.000826       & 0.000775           & 0.000784              & 6.2\%      \\
\midrule
\multicolumn{4}{c|}{\textbf{Average   improvement}}      &       \textbf{11.7}\% \\ 
\bottomrule
\end{tabular}
\label{tab:weatherbenchhmv}
}
% \end{sc}
\end{small}
\end{center}
% \vskip -0.3in
%\vspace{-5mm}
\end{table}



==> tables/tab_weatherbench_hmv2.tex <==
\begin{table}[H]
\centering
% \captionsetup{font=small} 
\caption{MAE comparison for SimVP and SVQ on WeatherBench-HMV (The last 55 channels).}
\begin{center}
% \vskip -0.2in
\begin{small}
% \begin{sc}
\scalebox{1}{
\begin{tabular}{c|c|c|c|c}
\toprule
Channel  & SimVP (w/o VQ) & SimVP+SVQ (Frozen) & SimVP+SVQ (Learnable) & Improvement \\
\midrule
q\_850   & 0.001054       & 0.000989           & 0.000994              & 6.1\%      \\
q\_925   & 0.0009         & 0.000757           & 0.00075               & 16.7\%     \\
q\_1000  & 0.001024       & 0.000776           & 0.000767              & 25.1\%     \\
t\_50    & 1.7426         & 1.2564             & 1.3594                & 27.9\%     \\
t\_100   & 1.5365         & 1.2852             & 1.3544                & 16.4\%     \\
t\_150   & 1.5825         & 1.3185             & 1.3377                & 16.7\%     \\
t\_200   & 1.7535         & 1.6099             & 1.6243                & 8.2\%      \\
t\_250   & 1.7895         & 1.5499             & 1.5571                & 13.4\%     \\
t\_300   & 1.5555         & 1.3903             & 1.3658                & 12.2\%     \\
t\_400   & 1.6055         & 1.4029             & 1.3737                & 14.4\%     \\
t\_500   & 1.6277         & 1.4652             & 1.4493                & 11.0\%     \\
t\_600   & 1.693          & 1.5669             & 1.5636                & 7.6\%      \\
t\_700   & 1.8961         & 1.7623             & 1.7412                & 8.2\%      \\
t\_850   & 2.1494         & 2.0246             & 1.8345                & 14.6\%     \\
t\_925   & 2.2241         & 1.8933             & 1.8747                & 15.7\%     \\
t\_1000  & 2.2335         & 1.891              & 1.834                 & 17.9\%     \\
u\_50    & 2.9882         & 2.5862             & 2.5981                & 13.5\%     \\
u\_100   & 3.4492         & 3.3665             & 3.3759                & 2.4\%      \\
u\_150   & 3.9731         & 3.7005             & 3.7262                & 6.9\%      \\
u\_200   & 4.8379         & 4.597              & 4.5959                & 5.0\%      \\
u\_250   & 5.725          & 5.5288             & 5.5195                & 3.6\%      \\
u\_300   & 5.9494         & 5.7551             & 5.7492                & 3.4\%      \\
u\_400   & 5.1291         & 4.9461             & 4.9373                & 3.7\%      \\
u\_500   & 4.2227         & 4.0826             & 4.0643                & 3.8\%      \\
u\_600   & 3.7165         & 3.6228             & 3.5999                & 3.1\%      \\
u\_700   & 3.4591         & 3.3916             & 3.3759                & 2.4\%      \\
u\_850   & 3.0929         & 3.0253             & 3.0211                & 2.3\%      \\
u\_925   & 2.9711         & 2.8879             & 2.8847                & 2.9\%      \\
u\_1000  & 2.3824         & 2.298              & 2.2888                & 3.9\%      \\
v\_50    & 2.4844         & 2.3521             & 2.346                 & 5.6\%      \\
v\_100   & 3.0661         & 2.9852             & 2.9837                & 2.7\%      \\
v\_150   & 3.8109         & 3.6697             & 3.6702                & 3.7\%      \\
v\_200   & 4.7779         & 4.6044             & 4.5961                & 3.8\%      \\
v\_250   & 5.6621         & 5.5064             & 5.4953                & 2.9\%      \\
v\_300   & 5.8984         & 5.7684             & 5.7591                & 2.4\%      \\
v\_400   & 5.0538         & 4.9421             & 4.9351                & 2.3\%      \\
v\_500   & 4.1298         & 4.0279             & 4.0228                & 2.6\%      \\
v\_600   & 3.612          & 3.5264             & 3.5224                & 2.5\%      \\
v\_700   & 3.3112         & 3.2528             & 3.2485                & 1.9\%      \\
v\_850   & 3.0267         & 2.9877             & 2.9857                & 1.4\%      \\
v\_925   & 2.9499         & 2.8942             & 2.8931                & 1.9\%      \\
v\_1000  & 2.3969         & 2.3354             & 2.3381                & 2.6\%      \\
vo\_50   & 8.64E-06       & 8.50E-06           & 8.50E-06              & 1.6\%      \\
vo\_100  & 1.16E-05       & 1.15E-05           & 1.15E-05              & 0.5\%      \\
vo\_150  & 1.59E-05       & 1.58E-05           & 1.58E-05              & 0.9\%      \\
vo\_200  & 2.26E-05       & 2.24E-05           & 2.24E-05              & 0.8\%      \\
vo\_250  & 3.24E-05       & 3.22E-05           & 3.22E-05              & 0.6\%      \\
vo\_300  & 3.85E-05       & 3.82E-05           & 3.82E-05              & 0.9\%      \\
vo\_400  & 3.61E-05       & 3.58E-05           & 3.57E-05              & 1.0\%      \\
vo\_500  & 2.99E-05       & 2.96E-05           & 2.96E-05              & 0.8\%      \\
vo\_600  & 2.69E-05       & 2.67E-05           & 2.68E-05              & 0.8\%      \\
vo\_700  & 2.68E-05       & 2.65E-05           & 2.65E-05              & 1.1\%      \\
vo\_850  & 2.76E-05       & 2.76E-05           & 2.76E-05              & 0.2\%      \\
vo\_925  & 2.64E-05       & 2.63E-05           & 2.63E-05              & 0.2\%      \\
vo\_1000 & 2.08E-05       & 2.08E-05           & 2.08E-05              & 0.1\%      \\
\midrule
\multicolumn{4}{c|}{\textbf{Average   improvement}}      &       \textbf{6.1}\% \\ 
\bottomrule
\end{tabular}
\label{tab:weatherbenchhmv2}
}
% \end{sc}
\end{small}
\end{center}
% \vskip -0.3in
%\vspace{-5mm}
\end{table}
